Reliable Transmission Spectrum Extraction with a Three-Parameter Limb Darkening Law

Stellar limb darkening must be properly accounted for to accurately determine the radii of exoplanets at various wavelengths. The standard approach to address limb darkening involves either using laws with coefficients from modelled stellar spectra or determining the coefficients empirically during light curve fitting of the data. Here, we test how accurately three common laws -- quadratic, power, and a three-parameter law -- can reproduce stellar limb darkening at different wavelengths and across a broad range of stars. We show that using a quadratic limb darkening law, which is most frequently employed by the community, leads to wavelength-dependent offsets in retrieved transmission spectra. For planets with high impact parameters ($b$ larger than about 0.5) the amplitude of these offsets can reach 1\% of the transit depth which is some cases is comparable to and can even exceed the expected signals from the planetary atmosphere. Furthermore, the quadratic law causes an offset in the value of the impact parameter when it is determined by fitting the broadband transit light curves. In contrast, using the Kipping--Sing three-parameter law leads to robust retrievals. We advocate the use of this law in retrievals, especially for transits with large impact parameters.

==> Main_points.tex <==
Simple list of main points to emphasise in the letter:
    - LDCs should be fit not fixed -> \citep{Espinoza2015}
        - Maybe mention large number of JWST papers still using this method, EXO-TiC specifically.
    - LDCs must be wavelength dependent -> no using white light LDCs for spectroscopic retrievals.
    -

    -Current work uses 1D stellar spectra; future work will use 3D MuRam simulations to examine these paramatrisations for more realistic models.
    

